Third-order accurate initialization of VOF volume fractions on unstructured meshes with arbitrary polyhedral cells

This paper introduces a novel method for the efficient and accurate computation of volume fractions on unstructured polyhedral meshes, where the phase boundary is an orientable hypersurface, implicitly given as the iso-contour of a sufficiently smooth level-set function. Locally, i.e. in each mesh cell, we compute a principal coordinate system in which the hypersurface can be approximated as the graph of an osculating paraboloid. A recursive application of the \textsc{Gaussian} divergence theorem then allows to analytically transform the volume integrals to curve integrals associated to the polyhedron faces, which can be easily approximated numerically by means of standard \textsc{Gauss-Legendre} quadrature. This face-based formulation enables the applicability to unstructured meshes and considerably simplifies the numerical procedure for applications in three spatial dimensions. We discuss the theoretical foundations and provide details of the numerical algorithm. Finally, we present numerical results for convex and non-convex hypersurfaces embedded in cuboidal and tetrahedral meshes, showing both high accuracy and third- to fourth-order convergence with spatial resolution.

==> 02_mathematical_details.tex <==
%
% Mathematical details
%
\section{Mathematical details}\label{sec:mathematical_details}%
Let $\cell*\subset\setR^3$ be an arbitrary polyhedron (cf.~subsection~\ref{subsec:notation}), intersected by a twice continuously differentiable oriented hypersurface $\iface$ with outer unit normal $\nS$, which is given as the zero iso-contour of a level-set function $\lvlset_\iface:\setR^3\mapsto\setR$ by %
\begin{align}
\iface=\set{\vx\in\setR^3:\lvlset_\iface\fofx=0}.\label{eqn:hypersurface_levelset}%
\end{align}
For obvious reasons, we assume that $\iface\cap\cell*\neq\emptyset$ and $\iface\not\subset\cell*$, i.e.\ the hypersurface intersects the boundary of the polyhedron $\cell*$. %
We are interested in the volume of the "interior" part of the polyhedron, i.e. %
\begin{align}
\cell\defeq\set{\vx\in\cell*:\lvlset_\iface\fofx\leq0},%
\end{align}
where the superscript "$-$" analogously applies to faces $\vfface_k$ and edges $\vfedge_{k,m}$. %
Henceforth, $\iface$ will be used to abbreviate $\iface\cap\cell*$ for ease of notation. %
Applying the \textsc{Gaussian} divergence theorem, the volume of an intersected polyhedron $\cell$ (cf.~\refeqn{problem_formulation}) can be cast as
\begin{align}
\abs{\cell}=\intcell{1}=\frac{1}{3}\brackets*[s]{\intdcell{\iprod{\vx-\xref}{\vn_{\partial\cell*}}}+\intiface{\iprod{\vx-\xref}{\nS}}},\label{eqn:volume_computation}%
\end{align}
where $\xref$ is an arbitrary but spatially fixed reference point. %; \reffig{intersection_quantities} illustrates the relevant quantities.
% %
% \begin{figure}[htbp]%
% \caption{Relevant quantities.}%
% \label{fig:intersection_quantities}%
% \end{figure}%
%
With some $\xiref\in\iface$, one may perform a change to the orthonormal base $\set{\vtau_1,\vtau_2,\vn_0}\fof{\xiref}$, where $\vn_0\defeq\nS\fof{\xiref}$ and $\vtau=\brackets[s]{\vtau_1,\vtau_2}$ are the unit normal and principal tangents%
\footnote{I.e., the tangents associated to the principal curvatures $\curv_i$, obtained from the \textsc{Weingarten} map.}%
 to $\iface$ at $\xiref$. %; cf.~\reffig{intersection_quantities} for an illustration. %
In the vicinity of $\xiref$, the inverse function theorem states that the hypersurface $\iface$ can be expressed as a graph of a height function; cf., e.g., the book of~\citet{Pruess2016}. In what follows, we assume that $\iface$ admits a unique explicit parametrization as %
\begin{align}
\iface=\set{\vf_\iface\fof{\vt}:\vt\in\support_\iface}\quad\text{with}\quad\vf_\iface\fof{\vt}=\xiref+\vtau\vt+h_\iface\fof{\vt}\vn_0,\qquad\evaluate{\frac{\partial h_\iface}{\partial\vt}}{\vt=\vec{0}}=\vec{0},%
\label{eqn:iface_map}%
\end{align}
and some parameter domain $\support_\iface\subset\setR^2$ (henceforth referred to as \textit{graph base}). The tangential coordinates associated to any $\vx\in\setR^3$ are obtained by the projection %
\begin{align}
\vt=\vtau\transpose\brackets{\vx-\xiref},\qquad\text{implying that}\qquad\support_\iface=\set{\vtau\transpose\brackets{\vx-\xiref}:\vx\in\iface}.\label{eqn:tangential_projection}%
\end{align}
%
% Integral transformation
%
Exploiting $\partial\cell\setminus\iface=\bigcup_{k}\vfface_k^-$ allows to cast the first summand in \refeqn{volume_computation} as %
\begin{align}
\intdcell{\iprod{\vx-\xref}{\vn_{\partial\cell*}}}%
=\sum\limits_{k}{\int_{\vfface_k^-}{\iprod{\vx-\xref}{\vn^\vfface_k}\darea}}%
=\sum\limits_{k}{\iprod{\vx_{k,1}^\vfface-\xref}{\vn^\vfface_k}\immersedarea{k}},\label{eqn:cell_boundary_contribution}%
\end{align}
corresponding to the sum of the immersed face areas $\immersedarea{k}\defeq\abs{\vfface_k^-}$, weighted by the signed distance $\iprod{\vx_{k,1}^\vfface-\xref}{\vn^\vfface_k}$ to the reference $\xref$. %
%
Inserting the explicit parametrization $\iface=\vf_\iface\fof{\support_\iface}$ given in \refeqn{iface_map}, the second summand in \refeqn{volume_computation} becomes %
\begin{align}
\intiface{\iprod{\vx-\xref}{\nS}}%&=%
%\intiface{\frac{\hiface-\iprod{\grad{\hiface}}{\vt}+\iprod{\xiref-\xref}{\vn_0-\vtau\grad{\hiface}}}{\sqrt{1+\iprod{\grad{}\hiface}{\grad{}\hiface}}}}\nonumber\\%
=\int_{\support_\iface}{\hat{h}_\iface\dd{\vt}}%
\quad\text{with}\quad%
\hat{h}_\iface\defeq\hiface-\iprod{\grad{\hiface}}{\vt}+\iprod{\xiref-\xref}{\vn_0-\vtau\grad{\hiface}}.%
\label{eqn:hypersurface_contribution}%
\end{align}
%
% Rationale
%
\begin{note}[Rationale]\label{note:rationale_normal}%
With the gradient $\grad{\hiface}\fof{\vt}\defeq\frac{\partial \hiface}{\partial\vt}$ of the height function and the functional determinant of the parametrization $\fundet{\vf_\iface}=\sqrt{1+\iprod{\grad{}\hiface}{\grad{}\hiface}}$, we obtain the normal according to %
\begin{align}
\nS=\frac{\vn_0-\vtau\grad{\hiface}}{\fundet{\vf_\iface}}.%
\end{align}
For any $\vx\in\iface$, it holds that $\vx-\xref=\xiref-\xref+\vtau\vt+\hiface\vn_0$, such that the inner product in the leftmost expression of \refeqn{hypersurface_contribution} becomes %
\begin{align}
\iprod{\vx-\xref}{\nS}=%
\frac{\hiface-\iprod{\grad{\hiface}}{\vt}+\iprod{\xiref-\xref}{\vn_0-\vtau\grad{\hiface}}}{\sqrt{1+\iprod{\grad{}\hiface}{\grad{}\hiface}}}%
=\frac{\hat{h}_\iface}{\fundet{\vf_\iface}},%
\label{eqn:hypersurface_contribution_reduced}%
\end{align}
where the integral transformation from $\iface$ to $\support_\iface$ then cancels the denomiator. %
\end{note}%
%
%
%
The continuity of $\hiface$ implies the existence of a function ("primitive") $\Hiface:\setR^2\mapsto\setR^2$ with $\div{\Hiface}=\hat{h}_\iface$. %
Applying the \textsc{Gaussian} divergence theorem once again, one obtains %
\begin{align}
\intiface{\iprod{\vx-\xref}{\nS}}=%
% \int_{\support_\iface}{\hiface\iprod{\grad{\hiface}}{\vt}\dd{\vt}}=%
\int_{\support_\iface}{\div{\Hiface}\dd{\vt}}=%
\int_{\partial\support_\iface}{\iprod{\Hiface}{\vn_{\support_\iface}}\dd{\vt}},%
\label{eqn:hypersurface_contribution_divergence}%
\end{align}
where $\vn_{\support_\iface}$ denotes the outer unit normal to the boundary of the graph base $\support_\iface$. %
Recall that, by assumption, the boundary $\partial\iface$ of the hypersurface is a subset of the polyhedron boundary, i.e.~$\partial\iface\subset\partial\cell*=\bigcup_k{\vfface_k}$. This suggests a decomposition based on the polyhedron faces $\vfface_k$. Let %
\begin{align}
\partial\iface=\bigcup\limits_{k}{\partial\iface_k}%
\qquad\text{with}\qquad%
\partial\iface_k=\partial\iface\cap\vfface_k=\vf_\iface\fof{\support_{\partial\iface,k}}%
\qquad\text{and}\qquad%
\support_{\partial\iface}=\bigcup\limits_{k}{\support_{\partial\iface,k}},%
\end{align}
which allows to rewrite the rightmost integral in \refeqn{hypersurface_contribution_divergence} as %
\begin{align}
\int_{\partial\support_\iface}{\iprod{\Hiface}{\vn_{\support_\iface}}\dd{\vt}}=%
\sum\limits_{k}{\int_{\partial\support_{\iface,k}}{\iprod{\Hiface}{\vn_{\support_\iface}}\dd{\vt}}}.%
\label{eqn:cell_hypersurface_contribution}%
\end{align}
Finally, combining \refeqs{cell_boundary_contribution} and \refeqno{cell_hypersurface_contribution} yields
\begin{align}
\abs{\cell}=\frac{1}{3}\brackets*[s]{\sum\limits_{k}{\iprod{\vx_{k,1}^\vfface-\xref}{\vn^\vfface_k}\immersedarea{k}+\int_{\support_{\partial\iface,k}}{\iprod{\Hiface}{\vn_{\support_\iface}}\dd{\vt}}}},\label{eqn:volume_computation_facebased}%
\end{align}
implying that the volume of a truncated polyhedral cell $\cell$ can be cast as the sum of face-based quantities (index $k$). %
%
%
%
While the inverse function theorem guarantees the existence of $\hiface$, its actual computation poses a highly non-trival task for general hypersurfaces. However, \refeqs{tangential_projection},\refeqno{hypersurface_contribution}--\refeqno{cell_hypersurface_contribution} and \refnote{rationale_normal} remain valid for an approximated hypersurface %
\begin{align}
\ifaceapprox=\set{\vf_\ifaceapprox\fof{\vt}:\vt\in\support_\ifaceapprox}\quad\text{with}\quad\vf_\ifaceapprox\fof{\vt}=\xiref+\vtau\vt+\happrox\fof{\vt}\vn_0,\label{eqn:ifaceapprox_map}%
\end{align}
where the notation introduced above for $\iface$ analogously applies to $\ifaceapprox$. %
The \textit{principal curvatures} $\curv_i$ and \textit{tangents} $\vtau_i$ at some $\xiref\in\iface$ induce a local second-order approximation %
\begin{align}
\happrox\fof{\vt}=\vt\transpose\vec{\curv}\vt=\frac{\curv_1t_1^2+\curv_2t_2^2}{2}%
=\hiface\fof{\vt}+\hot{\norm{\vt}^3}\qquad\text{with}\qquad%
\curvtensor=\frac{1}{2}\brackets*[s]{\begin{matrix}\curv_1&0\\0&\curv_2\end{matrix}},%
\label{eqn:hypersurface_approximation_quadratic}%
\end{align}
where for $\curv_i\equiv0$ one obtains a tangent plane; subsection~\ref{subsec:approximation_hypersurfaces} describes a procedure to obtain the parameters of the quadratic approximation. %
%
%
\begin{remark}[Non-principal approximation]%
The curvature tensor in \refeqn{hypersurface_approximation_quadratic} admits no off-diagonal elements, since it corresponds to a principal coordinate system. However, it is worth noting that the proposed algorithm can be readily extended to the non-principal case, i.e.~with non-zero diagonal elements $\curv_{12}=\curv_{21}$, by replacing \refeqn{hypersurface_approximation_quadratic} with %
\begin{align}
\happrox\fof{\vt}=\vt\transpose\vec{\curv}\vt=\frac{\curv_{11}t_1^2+2\curv_{12}t_1t_2+\curv_{22}t_2^2}{2}%
=\hiface\fof{\vt}+\hot{\norm{\vt}^3}\qquad\text{with}\qquad%
\curvtensor=\frac{1}{2}\brackets*[s]{\begin{matrix}\curv_{11}&\curv_{12}\\\curv_{12}&\curv_{22}\end{matrix}}%
\tag{\ref*{eqn:hypersurface_approximation_quadratic}$^\prime$}.%
\end{align}
\end{remark}%
%
Note that the hypersurface $\ifaceapprox$ in \refeqn{ifaceapprox_map} can also be expressed implicitly as the zero-isocontour of a level-set, i.e. %
\begin{align}
\ifaceapprox=\set{\vx\in\cell*:\lvlset_\ifaceapprox\fofx=0}%
\quad\text{with}\quad%
\lvlset_\ifaceapprox\fofx=\iprod{\vx-\xiref}{\vn_0}-\brackets{\vx-\xiref}\transpose\vtau\curvtensor\vtau\transpose\brackets{\vx-\xiref}.\label{eqn:ifaceapprox_lvlset}%
\end{align}%
%
\begin{assumption}[]%
In what follows, we focus on the non-trivial case in which at least one of the principal curvatures (say $\curv_1$) is nonzero. %
\end{assumption}%
%
For a hypersurface $\ifaceapprox$ of the above class, the integrand in \refeqn{hypersurface_contribution} becomes a third-order polynomial in $\vt$, namely %
\begin{align}
\hat{h}_\ifaceapprox&=h_0-\happrox+\iprod{\vec{\curv}\vec{\xi}}{\vt}\nonumber\\%
&=h_0-\frac{1}{2}\brackets*{\curv_1\brackets{t_1^2+2\xi_1t_1}+\curv_2\brackets{t_2^2+2\xi_2t_2}}%
\quad\text{with}\quad%
h_0\defeq\iprod{\xiref-\xref}{\vn_0}%
\quad\text{and}\quad%
\xi_i=-\iprod{\xiref-\xref}{\vtau_i}.\label{eqn:hypersurface_contribution_coefficients}%
\end{align}
Choosing the reference point to coincide with the paraboloid base point, i.e.~$\xref\defeq\xiref$, implies $h_0=\xi_i=0$. For reasons that will become clear below, we choose the primitive %
\begin{align}
\Happrox\defeq\ve_1\int{\hat{h}_\ifaceapprox\dd{t_1}}%
% &=\ve_1\brackets*[s]{h_0t_1-\frac{1}{6}\brackets*{\curv_1\brackets{t_1^3+3\xi_1t_1^2}+3\curv_2t_1\brackets{t_2^2+2\xi_2t_2}}}+C_0(t_2)\nonumber\\%
% &=\frac{\ve_1}{6}\brackets*[s]{6h_0t_1-\curv_1\brackets{t_1^3+3\xi_1t_1^2}-3\curv_2t_1\brackets{t_2^2+2\xi_2t_2}}+C_0(t_2).\\%
% &=-\frac{\ve_1}{6}\brackets*[s]{\curv_1t_1^3+3\curv_1\xi_1t_1^2+3\curv_2t_1\brackets{t_2^2+2\xi_2t_2-2h_0}}+C_0(t_2).%
=-\frac{\ve_1}{6}\hat{H}_\ifaceapprox%
\quad\text{with}\quad%
\hat{H}_\ifaceapprox\defeq\curv_1t_1^3+3\curv_2t_1t_2^2.%
\label{eqn:hypersurface_primitive_paraboloid}%
\end{align}
% corresponding to an integral of a polynomial over a planar domain with piecewise smooth boundary
%
%
%
\begin{note}[The choice of the reference point $\xref$]%
On the one hand, choosing $\xref\defeq\xiref$ apparently implies $h_0=\xi_i=0$ in \refeqn{hypersurface_contribution_coefficients}, implying that the evaluation of \refeqn{hypersurface_primitive_paraboloid} involves fewer multiplications\footnote{The exact gain in efficiency depends, among others, on the compiler options as well the evaluation scheme, e.g., \textsc{Horner}.}. However, $\xiref$ will in general not be coplanar to any of the faces $\vfface_k$, such that the associated immersed areas $\immersedarea{k}$ have to be computed. %
One the other hand, a polyhedral cell $\cell*$ intersected\footnote{Note that, by definition, \textit{intersected} means that the polyhedron $\cell*$ admits at least one interior and one exterior vertex; cf.~\ref{}.} by a paraboloid admits at least three intersected faces. Out of those, at least two, say $\vfface_{k_1}$ and $\vfface_{k_2}$, share a common vertex, implying that the respective containing planes intersect, i.e.~$\abs{\iprod{\vn^\vfface_{k_1}}{\vn^\vfface_{k_2}}}\neq1$. %
While choosing $\xref$ to be coplanar to $\vfface_{k_1}$ and $\vfface_{k_2}$ avoids computing the immersed areas $\immersedarea{k_1}$ and $\immersedarea{k_2}$, the evaluation of \refeqn{hypersurface_primitive_paraboloid} becomes more costly in terms of floating point operations. %
Since the evaluation has to be carried out for all intersected faces, irrespective of the choice of the reference point $\xref$, cf.~\refeqn{volume_computation_facebased}, the most efficient choice can only be substantiated by numerical experiments. %
\end{note}
%Choose $\xref$ to be the first intersection on some edge. By doing so, the two faces $\set{\vfface_{k_1},\vfface_{k_2}}$ containing $\xref$ do not contribute to the integral, implying a gain of efficiency by skipping the computation of the associated immersed areas $\immersedarea{k}$. %
Replacing the original hypersurface $\iface$ in \refeqn{volume_computation_facebased} by the locally parabolic approximation $\ifaceapprox$ yields the approximative enclosed volume %
\begin{align}
\abs{\cell}\approx\frac{1}{3}\brackets*[s]{\sum\limits_{k}{\iprod{\vx_{k,1}^\vfface-\xref}{\vn^\vfface_k}\immersedarea{k}+%
\int_{\partial\support_{\ifaceapprox,k}}{\iprod{\Happrox}{\vn_{\support_\ifaceapprox}}\dd{\vt}}}}.\label{eqn:volume_computation_facebased_approx}%
\end{align}
Since \refeqn{volume_computation_facebased_approx} expresses the enclosed volume as a sum of face-based quantities, in what follows we focus on a single intersected face $\vfface_k$ of the polyhedron. Before the numerical evaluation of the right-hand side of \refeqn{volume_computation_facebased_approx} can be addressed componentwise, the upcoming subsections discuss the local approximation of hypersurfaces and introduce a classification of the boundary segments $\partial\ifaceapprox_k=\ifaceapprox\cap\vfface_k$. %
%
% Local approximation of hypersurfaces
%
\subsection{A local approximation of the hypersurface $\iface$}\label{subsec:approximation_hypersurfaces}%
In order to obtain a base point $\xiref\in\iface$, on each edge $\vfedge_{k,m}$ we approximate the level-set $\lvlset_\iface$ by a cubic polynomial based on the values and gradient of the level-set evaluated at its respective vertices, i.e.~$\lvlset_\iface\fof{\vx^\vfface_{k,m}}$ and $\grad{\lvlset_\iface}\fof{\vx^\vfface_{k,m}}$. %
Note that, in this part of the algorithm, an edge will only be considered \textit{intersected} iff $\lvlset_\iface\fof{\vx^\vfface_{k,m}}\lvlset_\iface\fof{\vx^\vfface_{k,m+1}}<0$, i.e.~if the level-set admits a sign change along the edge $\vfedge_{k,m}$. If existent, the associated root $\vx^\iface_{k,m}$ is computed numerically using a standard \textsc{Newton} scheme. %
%
\begin{note}[Logical intersection status]%
Technically, deducing the logical intersection status of $\vfface_k$ from the level-set values is not possible for general hypersurfaces. E.g., a face $\vfface_k$ whose vertices $\vx^\vfface_{k,m}$ are entirely located in the negative halfspace of $\iface$ (i.e., $\lvlset_\iface\fof{\vx^\vfface_{k,m+1}}<0$ $\forall m$) may still admit intersections with the positive halfspace of $\iface$. Hence, care has to be taken for the status assignment on the hierarchically superior cell level. In what follows, we assume that the spatial resolution of the underlying mesh is sufficient to capture all geometrical details, implying that each intersected cell contains at least one intersected edge that admits a sign change of the level-set $\lvlset_\iface$. %
\end{note}%
%
The base point $\xiref\in\iface$ then results from a metric projection of the average of all approximate intersections $\set{\vx^\iface_{k,m}}$ onto the hypersurface $\iface$. %
Finally, the paraboloid parameters in \refeqn{ifaceapprox_map}, namely the normal $\vn_0\defeq\nS\fof{\xiref}$, principal tangents $\vtau\defeq\vtau_\iface\fof{\xiref}$ and curvature tensor $\curvtensor\defeq\curvtensor_\iface\fof{\xiref}$ can be obtained from the \textsc{Weingarten} map. %
\begin{note}[Approximation quality]%
\label{note:approximation_quality}%
The choice of the reference point $\xiref$ crucially affects the global (with respect to the cell) approximation quality, measured by the symmetric volume difference (red hatched). \\%
\null\hfill%
\includegraphics[page=1]{approximation_error}%
\hfill%
\includegraphics[page=3]{approximation_error}%
\hfill%
\includegraphics[page=2]{approximation_error}%
\hfill\null%
\\%
Under mild restrictions, intuition suggests to select a reference point $\xiref$ close to the (loosely speaking) "center" of the enclosed hypersurface patch, which aims at reducing the effect of the quadratic growth of the deviation by choosing a reference point whose distance to the boundary is as uniform as possible. In fact, this is the motivation behind the metric projection applied here, which has been shown to produce decent results \cite{JCP_2019_haco}. %
However, as can be seen from the rightmost panel, this is not necessarily the "best" choice. At this point, note that even the formulation of a minimization problem for general hypersurfaces and polyhedra poses a highly non-trivial task, let alone finding a minimum. Beyond that, due to the cell-wise application, computing such a minimum likely imposes considerable computational effort. %
\end{note}%
%
% Computation of edge intersections
%
\subsection{Intersections of edges $\vfedge_{k,m}$ and paraboloids $\ifaceapprox$}\label{subsec:computation_edge_intersections}%
The intersection of an edge and a paraboloid is conducted in the following way: %
Let the edge $\vfedge_{k,m}$ be parametrized as $$\vfedge_{k,m}=\set*{\vx^\vfface_{k,m}+v\brackets{\vx^\vfface_{k,m+1}-\vx^\vfface_{k,m}}:v\in[0,1]}.$$ %
Due to the quadratic character of the paraboloid, the associated level-set can be expressed as a second-order polynomial in the edge coordinate $v$. Employing the level-set from \refeqn{ifaceapprox_lvlset}, one obtains %
\begin{align}
\lvlset^\vfedge_{k,m}\fof{v}=&%
\brackets*{\lvlset_\ifaceapprox\fof{\vx^\vfface_{k,m+1}}-\lvlset_\ifaceapprox\fof{\vx^\vfface_{k,m}}-\iprod{\vx^\vfface_{k,m+1}-\vx^\vfface_{k,m}}{\grad{\lvlset_\ifaceapprox}\fof{\vx^\vfface_{k,m}}}}v^2+\nonumber\\%
&\brackets*{\iprod{\vx^\vfface_{k,m+1}-\vx^\vfface_{k,m}}{\grad{\lvlset_\ifaceapprox}\fof{\vx^\vfface_{k,m}}}}v+%
\lvlset_\ifaceapprox\fof{\vx^\vfface_{k,m}}.\label{eqn:ifaceapprox_levelset_edge}%
\end{align}
\refEqn{ifaceapprox_levelset_edge} exhibits $0\leq N^\ifaceapprox_{k,m}\leq2$ real roots $\set{v^\ifaceapprox_{k,m,i}}\subset(0,1)$, to which we associate the intersections $\vx^\ifaceapprox_{k,i}$; cf.~\reffig{intersection_ordering} for an illustration. If two roots are present, we assume without loss of generality that $1>v^\ifaceapprox_{k,m,2}\geq v^\ifaceapprox_{k,m,1}>0$. %
The details of the computation of the relative immersed lengths $\immersedlength{k}{m}$ associated to edge $\vfedge_{k,m}$ can be found in \reftab{immersed_length_edge}. %
%
\begin{table}[htbp]%
\caption{Relative immersed length $\immersedlength{k}{m}$ (red) on edge $\vfedge_{k,m}$ (gray) intersected by with parabola $\lvlset^\vfedge_{k,m}$; cf.~\protect\refeqn{ifaceapprox_levelset_edge}.}%
\label{tab:immersed_length_edge}%
\centering%
\renewcommand{\arraystretch}{1.5}%
\begin{tabular}{|c||c|c|c|}%
\multicolumn{4}{c}{}\\%
\hline
&$N^\ifaceapprox_{k,m}=0$&$N^\ifaceapprox_{k,m}=1$&$N^\ifaceapprox_{k,m}=2$\\%
\hline\hline%
$\lvlset^\vfedge_{k,m}\fof{0}<0$&$0$&$1-v^\ifaceapprox_{k,m,1}$&$v^\ifaceapprox_{k,m,2}-v^\ifaceapprox_{k,m,1}$\\%
&\includegraphics[page=4]{roots_on_edge}&\includegraphics[page=5]{roots_on_edge}&\includegraphics[page=1]{roots_on_edge}\\%
\hline%
$\lvlset^\vfedge_{k,m}\fof{0}>0$&$1$&$v^\ifaceapprox_{k,m,1}$&$1-v^\ifaceapprox_{k,m,2}+v^\ifaceapprox_{k,m,1}$\\%
&\includegraphics[page=3]{roots_on_edge}&\includegraphics[page=6]{roots_on_edge}&\includegraphics[page=2]{roots_on_edge}\\%
\hline%
\end{tabular}%
\end{table}%
%

Each intersection $\vx^\ifaceapprox_{k,i}$ can be classified based on the sign of $\evaluate{\partial_v\lvlset^\vfedge_{k,m}}{v=v_{0,i}}$ as either \textit{entering} (negative) or \textit{leaving} (positive), providing a key information for establishing the topological connectivity required for the computation of immersed areas $\immersedarea{k}$ in subsection~\ref{subsec:topological_connectivity}. %
%
Note that the total number of intersections on each face $\vfface_k$ is even\footnote{Intersected vertices must hence be either considered twice or not all all.} and corresponds to twice the number of curved segments $M_k$, i.e.~$2M_k=\sum_{m=1}^{N^\vfface_k}{N^\ifaceapprox_{k,m}}$. %
Furthermore, the sequence of intersections $\set{\vx^\ifaceapprox_{k,m}}$ alternates between \textit{entering} and \textit{leaving} if the edges $\vfedge_{k,m}$ of the face are traversed in counter-clockwise order with respect to the face normal $\vn^\vfface_k$. %
%
% Transformation to principal coordinates
%
\subsection{Transformation to principal coordinates}\label{subsec:transformation_principal_coordinates}%
The robust treatment of the curved segments $\partial\ifaceapprox_k$ calls for a classification of the intersection curves in terms of locally principal coordinates; cf.~\reftab{possible_curve_class}. %
Let the polyhedron face $\vfface_k$ be parametrized as %
\begin{align}
\vfface_k=\set{\vx^\vfface_{k,1}+\vmu_k\vu:\vu\in\support_{\vfface,k}}%
\quad\text{with}\quad%
\vmu_k=\brackets[s]{\vmu_{k,1},\vmu_{k,2}},\quad%
\vmu_k\transpose\vmu_k=\ident,\quad%
\vmu_k\transpose\vn^\vfface_k=\vec{0},%
\label{eqn:cell_face_parametrization}%
\end{align}
and some parameter domain $\support_{\vfface,k}\subset\setR^2$. %
We apply the tangential projection from \refeqn{tangential_projection} to the map given in \refeqn{cell_face_parametrization} and plug the result into \refeqn{ifaceapprox_map} to obtain the implicit quadratic definition of the boundary curve segment $\partial\ifaceapprox_k=\ifaceapprox\cap\vfface_k$, namely %
\begin{align}
\partial\ifaceapprox_k=\set{\vu\in\support_{\vfface,k}:\iprod{\vu}{\tA_k\vu}+\iprod{\vu}{\va_k}+a_k=0}%
\label{eqn:support_levelset_definition}%
\end{align}
with the coefficients %
\begin{align}
a_k=\iprod{\vx^\vfface_{k,1}-\xiref}{\vtau\curvtensor\vtau\transpose\brackets{\vx^\vfface_{k,1}-\xiref}-\vn_0},\quad%
\va_k=\vmu_k\transpose\brackets*{2\vtau\curvtensor\vtau\transpose\brackets{\vx^\vfface_{k,1}-\xiref}-\vn_0}\quad\text{and}\quad%
\tA_k=\vmu_k\transpose\vtau\curvtensor\vtau\transpose\vmu_k.\!\!%
\end{align}
\refTab{possible_curve_class} gathers and illustrates the admissible curve classes that emerge from \refeqn{support_levelset_definition}. %
%
\begin{table}[htbp]%
\centering%
\renewcommand{\arraystretch}{1.25}%
\caption{Classification of intersections $\partial\ifaceapprox_k$ (red) of planar faces $\vfface_k$ (red shaded) and paraboloids $\ifaceapprox$ (blue). Note that the linear case requires the tangential plane and the face to intersect orthogonally.}%
\label{tab:possible_curve_class}%
\begin{tabular}{l|c|c|c|c}
\multicolumn{5}{c}{}\\%
&\textbf{hyperbolic}&\textbf{elliptic}&\textbf{parabolic}&\textbf{linear}\\%
&\includegraphics[width=3cm,page=1]{curve_classes}%
&\includegraphics[width=3cm,page=3]{curve_classes}%
&\includegraphics[width=3cm,page=2]{curve_classes}%
&\includegraphics[width=3cm,page=4]{curve_classes}\\%
\hline%
$\textcolor{black}{0<}\abs{\iprod{\vn^\vfface_k}{\vn_0}}\leq1$&\cellcolor{black!25}$\curv_1\curv_2<0$&%
\cellcolor{black!25}$\curv_1\curv_2>0$&\cellcolor{black!25}$\begin{matrix}\curv_1\curv_2=0\\\curv_1+\curv_2\neq0\end{matrix}$&\\%
\hline%
$\phantom{0<}\abs{\iprod{\vn^\vfface_k}{\vn_0}}=0$&&&\cellcolor{black!25}$\curv_1\curv_2\lesseqqgtr0$&\cellcolor{black!25}$\curv_1\curv_2=0$%
\end{tabular}
\end{table}
%

Note that the matrix of quadratic coefficients $\tA_k$ will not admit diagonal form in general. %
With%
\footnote{The proof of this statement employs that, by definition, we have $\norm{\vmu_{k,1}}=\norm{\vmu_{k,2}}=1$, $\iprod{\vmu_{k,1}}{\vmu_{k,2}}=0$ and $\iprod{\vtau_1}{\vtau_2}=0$. %
Expanding the $i$-th row of $\vtau\transpose\vmu_k=\vec{0}$ yields $\iprod{\vtau_i}{\vmu_1}=\iprod{\vtau_i}{\vmu_2}=0$, implying that %
$\vtau_i=\beta_i\brackets{\cross{\vmu_1}{\vmu_2}}=\beta_i\vn^\vfface_k$ with some $\beta_i\in\setR\setminus\set{0}$. In combination, one obtains the contradiction $\iprod{\vtau_1}{\vtau_2}=\beta_1\beta_2\neq0$.} %
$\vtau\transpose\vmu_k\neq\vec{0}$, the principal coordinates $\vu^\prime$ emerge from $\vu$ via %
\begin{align}
\vu=\tensor[2]{R}_k\transpose\vu^\prime+\vu_{0,k}%
\quad\text{with}\quad%
\tensor[2]{R}_k=\brackets*[s]{\begin{matrix}\cos\psi_k&\sin\psi_k\\-\sin\psi_k&\cos\psi_k\end{matrix}}%
\quad\text{and}\quad%
\tan2\psi_k=\frac{2A_{k,12}}{A_{k,11}-A_{k,22}}.%
\label{eqn:principal_face_coordinates}%
\end{align}
For notational convenience, let $\vr_{i,k}=\tensor[2]{R}_k\transpose\ve_i$. %
With \refeqn{principal_face_coordinates}, the quadratic equation in \refeqn{support_levelset_definition} can be rewritten as %
\begin{align}
\iprod{\vu^\prime}{\tensor[2]{B}_k\vu^\prime}+\iprod{\vu^\prime}{\vb_k}+b_k=0%
%
\label{eqn:support_levelset_definition_principal}%
\end{align}
with the coefficients  %
\begin{align}
b_k=a_k+\iprod{\vu_{0,k}}{\va_k+\tA_k\vu_{0,k}},%
\quad%
\vb_k=\tensor[2]{R}_k\brackets{\va_k+2\tA_k\vu_{0,k}}%
\quad\text{and}\quad%
\tensor[2]{B}_k=\tensor[2]{R}_k\tA_k\tensor[2]{R}_k\transpose=\diag{B_{k,1},B_{k,2}}.%
\label{eqn:support_levelset_definition_principal_coeff}%
\end{align}
The eigenvalues of $\tensor[2]{B}_k$ ($B_{k,1}\geq B_{k,2}$) classify the boundary segment $\partial\ifaceapprox_k$: %
\begin{enumerate}
% elliptic and hyperbolic
\item For $\det\tensor[2]{B}_k\neq0$, the curve segment is \textit{elliptic} ($\det\tensor[2]{B}_k>0$) or \textit{hyperbolic} ($\det\tensor[2]{B}_k<0$). In both cases, the coefficients in \refeqn{support_levelset_definition_principal_coeff} read %
\begin{align}
\vb_k=\vec{0}%
\quad\text{and}\quad%
b_k=a_k+\frac{\iprod{\va_k}{\vu_{0,k}}}{2}%
\quad\text{with the origin}\quad%
\vu_{0,k}=-\frac{1}{2}\tA_k\inverse\va_k.%
\label{eqn:curveclass_det_nonzero}%
\end{align}
%
% parabolic
%
\item For $\det{\tensor[2]{B}_k}=\det{\tA_k}=0$, the curve segment is either \textit{parabolic} ($B_{k,1}\neq0$, $B_{k,2}=0$) or \textit{linear} ($B_{k,1}=B_{k,2}=0$). %
For parabolic intersections, exploiting that $\iprod{\vr_{2,k}}{\tA_k\vr_{2,k}}=B_{k,2}=0$ yields %the coefficents in \refeqn{support_levelset_definition} in become %
% \begin{align}
% % \iprod{\vu^\prime}{\tB_k\vu^\prime}+\iprod{\vu^\prime}{\tensor[2]{R}_k\va_k}+a_k+w\iprod{\va_k}{\vec{\beta}_k}=0.%
% \iprod{\vu^\prime}{\tB_k\vu^\prime}+\iprod{\vu^\prime}{\tensor[2]{R}_k\va_k}=0.%
% \end{align}
\begin{align}
\vb_k=\tensor[2]{R}_k\va_k%
\quad\text{and}\quad%
b_k=0%
\quad\text{with the origin}\quad%
\vu_{0,k}=%
\begin{cases}%
-\frac{a_k}{\iprod{\va_k}{\vr_{2,k}}}\vr_{2,k}&\text{if}\quad\iprod{\va_k}{\vr_{2,k}}\neq0,\\%
-\frac{\iprod{\va_k}{\vr_{1,k}}}{2B_{k,1}}\vr_{1,k}&\text{if}\quad\iprod{\va_k}{\vr_{2,k}}=0.%
\end{cases}%
\label{eqn:curveclass_det_zero}%
\end{align}
In the second case of \refeqn{curveclass_det_zero}, the intersection consists of two parallel lines. While this corresponds to a parabola whose vertex is located at infinity, we prefer a treatment as a degenerate hyperbola for consistency of implementation. %
%
%
%
For linear intersections ($B_{k,1}=B_{k,2}=0$), one obtains %
\begin{align}%
\vb_k=\tensor[2]{R}_k\va_k%
\quad\text{and}\quad%
b_k=a_k%
\quad\text{with the origin}\quad%
\vu_{0,k}=\vec{0}.%
\end{align}%
\end{enumerate}
%
% Explicit curve parametrization
%
With the curve parameter $s$, the above classification induces the following explicit parametrizations: %
\begin{align}
\vu_k^\prime\fof{s}=%
\begin{cases}
\brackets*[s]{\sqrt{\frac{-B_{k,1}}{b_k}}\cos s,\sqrt{\frac{-B_{k,2}}{b_k}}\sin s}\transpose&\text{elliptic},\\%
\brackets*[s]{\pm\sqrt{-\frac{b_k+B_{k,2}s^2}{B_{k,1}}},s}\transpose&\text{hyperbolic},\\%
\brackets*[s]{s,\frac{\iprod{\va_k}{\vr_{1,k}}}{\iprod{\va_k}{\vr_{2,k}}}s+\frac{B_{k,1}}{\iprod{\va_k}{\vr_{2,k}}}s^2}\transpose&\text{parabolic},\\%
\brackets*[s]{s\sin\varphi_k-b_k\cos\varphi_k,-s\cos\varphi_k-b_k\sin\varphi_k}\transpose&\text{linear with }\tan\varphi_k=\frac{\iprod{\va_k}{\vr_{2,k}}}{\iprod{\va_k}{\vr_{1,k}}}.%
\end{cases}
\label{eqn:parametrization_curve_class}%
\end{align}
By plugging \refeqn{parametrization_curve_class} into \refeqn{principal_face_coordinates}, one obtains an explicit parametrization of the boundary segment, i.e. %
\begin{align}%
\partial\ifaceapprox_k=%
\set*{\vx^\vfface_{k,1}+\tensor[2]{\mu}_k\brackets*{\vu_{k,0}+\tensor[2]{R}_k\vu_k^\prime\fof{s}}:s\in\support_{\partial\ifaceapprox,k}}%
\quad\text{with}\quad%
\support_{\partial\ifaceapprox,k}=\bigcup_{m=1}^{M_k}\brackets[s]{s_{k,2m-1}^\ifaceapprox,s_{k,2m}^\ifaceapprox},%
\label{eqn:boundary_curve_principal_coordinates}%
\end{align}
where the union over $M_k$ (number of curved segments of $\partial\vfface_k^-$) intervals reflects the fact that $\partial\ifaceapprox_k$ is not necessarily simply connected; cf.~the rightmost panel in \reffig{face_intersection_elliptic_hyperbolic}. %
%
The interval boundaries $s_{k,m}^\ifaceapprox$ are obtained by first projecting the edge intersections $\vx^\ifaceapprox_{k,m}$ (cf.~subsection \ref{subsec:computation_edge_intersections}) onto the principal coordinates of face $\vfface_k$ via %
\begin{align}
\vu^\prime_{k,m}=\tensor[2]{R}_k\brackets*{\tensor[2]{\mu}_k\transpose\brackets*{\vx^\ifaceapprox_{k,m}-\vx^\vfface_{k,1}}-\vu_{0,k}}%
\end{align}
and subsequent inversion of the respective parametrization in \refeqn{parametrization_curve_class}. %
%
% Projection to the
%
Projecting the map in \refeqn{boundary_curve_principal_coordinates} onto the base plane of the paraboloid $\ifaceapprox$ using \refeqn{tangential_projection} yields %
\begin{align}
\partial\support_{\ifaceapprox,k}=%
\set{\vt_{0,k}+\tensor[2]{T}_{0,k}\vu_k^\prime\fof{s}:s\in\support_{\partial\ifaceapprox,k}}%
\quad\text{with}\quad%
\vt_{0,k}\defeq\vtau\transpose\brackets{\vx^\vfface_{k,1}-\xiref+\tensor[2]{\mu}_k\vu_{k,0}}%
\quad\text{and}\quad%
\tensor[2]{T}_{0,k}\defeq\vtau\transpose\tensor[2]{\mu}_k\tensor[2]{R}_k,%
\label{eqn:boundary_support_segment}%
\end{align}
corresponding to the integration domain required for the evaluation of \refeqn{volume_computation_facebased_approx}. %
From \refeqn{boundary_support_segment}, the boundary normals are obtained via %
\begin{align}
\vn_{\support_{\ifaceapprox,k}}=%
%\brackets*[s]{\begin{matrix}0&-1\\1&0\end{matrix}}%
\brackets*[s]{\ve_2,-\ve_1}%
\frac{\tensor[2]{T}_{0,k}\partial_s\vu_k^\prime}%
{\sqrt{\iprod{\tensor[2]{T}_{0,k}\partial_s\vu_k^\prime}{\tensor[2]{T}_{0,k}\partial_s\vu_k^\prime}}},%
\quad\text{where}\quad%
\iprod*{\vn^\vfface_k-\frac{\iprod{\vn^\vfface_k}{\grad{\lvlset_\ifaceapprox}}}{\iprod{\grad{\lvlset_\ifaceapprox}}{\grad{\lvlset_\ifaceapprox}}}\grad{\lvlset_\ifaceapprox}}{\vtau\vn_{\support_\ifaceapprox,k}}\stackrel{!}{>}0%
\label{eqn:boundary_support_outer_normal}%
\end{align}
must be enforced by, e.g., sign inversion to ensure that $\vn_{\support_{\ifaceapprox,k}}$ is an outer normal to $\support_\ifaceapprox$; cf.~\reffig{illustration_graphbase} for an illustration. %
Recall from \refeqn{hypersurface_primitive_paraboloid} that, by design, $\iprod{\Happrox}{\ve_2}\equiv0$. This allows to rewrite the second summand in \refeqn{volume_computation_facebased_approx} as %
\begin{align}
\int\limits_{\partial\support_{\ifaceapprox,k}}{\iprod{\Happrox}{\vn_{\support_\ifaceapprox}}\dd{\vt}}=%
-\sum\limits_{m=1}^{M_k}{\int\limits_{s_{k,2m-1}^\ifaceapprox}^{s_{k,2m}^\ifaceapprox}{\ve_2\transpose\tensor[2]{T}_{0,k}\partial_s\vu_k^\prime\fof{s}\hat{H}_\ifaceapprox\fof{\vt_k\fof{s}}\dd{s}}}%
\quad\text{with}\quad%
\vt_k\fof{s}=\vt_{0,k}+\tensor[2]{T}_{0,k}\vu_k^\prime\fof{s},%
\label{eqn:quadrature_line_integral}%
\end{align}
which will be evaluated by standard \textsc{Gauss-Legendre} quadrature using $N_{\mathrm{quad}}=5$ nodes. %
%
\begin{figure}[htbp]
\null\hfill%
\includegraphics{cube_example}%
\hfill%
\includegraphics{cube_boundarycurve_paradom}%
\hfill\null%
\caption{Illustration of intersected hexahedral cell with associated graph base $\support_\ifaceapprox$.}%
\label{fig:illustration_graphbase}%
\end{figure}

%
%
%
\subsection{Topological connectivity of curve segments}\label{subsec:topological_connectivity}%
\label{subsec:topological_connectivity}%
The logical status of the principal origin $\vu_{k,0}$, denoted $\vfstatus{}_k$, induces the correct orientation for elliptic, hyperbolic and linear curve segments. In the parabolic case, the origin $\vu_{k,0}$ is located on the curve segment. Hence, one needs to consider the focus point to assess the orientation ($\textcolor{blue}{\blacksquare}$ in the bottom left panel in \reffig{intersection_ordering}). One obtains %
\begin{align}%
\vfstatus{}_k=%
\begin{cases}%
-\sign{b_k}&\text{elliptic/hyperbolic/parabolic (degenerate)},\\%
-\sign{a_k}&\text{linear},\\%
\phantom{-}\sign{B_{k,1}}&\text{parabolic}.%
\end{cases}
\label{eqn:logical_status_center}%
\end{align}%
%
For elliptic\footnote{A proper implementation of the arcus tangens ensures that the transition of the numerical values for the angles at $0$ and $2\pi$ is handled correctly.}, parabolic and linear segments on \textbf{convex} faces $\vfface_k$, traversing the edges $\vfedge_{k,m}$ counter-clockwise with respect to the normal $\vn^\vfface_k$, yields a properly ordered sequence of intersections $\set{\vx^\ifaceapprox_{k,m}}$. %
Hyperbolic segments additionaly require to first assign the intersections to the respective branch of the hyperbola (cyan/blue in the top left panel of \reffig{intersection_ordering}). For an exterior center $\vu_{0,k}$ ($\vfstatus{}_k=+1$ in \refeqn{logical_status_center} and $\square$ in \reffig{intersection_ordering}), the order of the sequence center must be inverted. %
%
After the intersections have been arranged in this manner, one needs to ensure that the first intersection is of type \textit{entering} by possibly performing an index shift\footnote{Note that the direction of the shift is irrelevant for our purpose. However, we shift to the left, i.e.~$\vx^\ifaceapprox_{k,m}\mapsto\vx^\ifaceapprox_{k,m-1}$ for all $m$.}. \refFig{intersection_ordering} illustrates the concept. %
%
\begin{figure}[htb]%
\null\hfill%
\includegraphics[page=5]{boundary_curve_ordering}%
\hfill%
\includegraphics[page=3]{boundary_curve_ordering}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=1]{boundary_curve_ordering_annotation}%
\hfill%
\includegraphics[page=5]{boundary_curve_ordering_annotation}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=2]{boundary_curve_ordering_annotation}%
\hfill%
\includegraphics[page=6]{boundary_curve_ordering_annotation}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=1]{boundary_curve_ordering}%
\hfill%
\includegraphics{boundary_curve_ordering_nonconvex}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=3]{boundary_curve_ordering_annotation}%
\hfill%
\includegraphics[page=1]{boundary_curve_ordering_nonconvex_annotation}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=4]{boundary_curve_ordering_annotation}%
\hfill%
\includegraphics[page=2]{boundary_curve_ordering_nonconvex_annotation}%
\hfill\null%
%
\caption{Intersection ordering for different curve classes (hyperbolic/convex, elliptic/convex, parabolic/convex and elliptic/non-convex) with initial (top) and sorted (bottom) list of intersections.}%
\label{fig:intersection_ordering}%
\end{figure}
%
\begin{remark}[Non-convex faces $\vfface_k$]%
As can be seen from the bottom right panel in \reffig{intersection_ordering}, non-convex faces potentially degrade the immanent order of intersections. %
Hence, the correct order of the intersections can be established be arranging the curve parameters $s^\pm_{k,m}$ associated to $\vx^\ifaceapprox_{k,m}$ (cf.~\refeqn{parametrization_curve_class}) in an ascending/descending order. %
\end{remark}%
For the remainder of this manuscript, we assume that the intersections $\set{\vx^\ifaceapprox_{k,m}}$ are arranged in the above manner. %
%
%
%
%
\subsection{Computation of immersed areas $\immersedarea{k}$}%
In a manner similar to \refeqn{volume_computation}, the boundary of an immersed face $\vfface_k^-$ can be decomposed into linear and curved segments, where the latter respectively connect two edge intersections. %
For each curved segment, we introduce an edge $\vfedge^\ifaceapprox_{k,m}$ (green in the center panel of \reffig{face_decomposition}) that connects the associated intersections. In other words, we (i) replace the curved segments by lines to form a (set of) polygons and (ii) connect the end points of the removed curved segments to form closed paths confining curved caps. %
%
\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=1]{boundary_face_decomposition}%
\hfill%
\includegraphics[page=2]{boundary_face_decomposition}%
\hfill%
\includegraphics[page=3]{boundary_face_decomposition}%
\hfill\null%
\caption{Decomposition of immersed face $\vfface_k^-$ into polygonal (center) and non-polygonal (right) part.}%
\label{fig:face_decomposition}%
\end{figure}%

This implies that the immersed area $\immersedarea{k}$ is fed from two contributions: %
\begin{enumerate}%
\item The \textbf{polygonal} part can be computed from two sets of edges: (i) the immersed segments of the original edges $\vfedge^-_{k,m}$, which we represent by the original edge $\vfedge_{k,m}$ and its associated relative immersed length $\immersedlength{k}{m}$ (cf.~\reftab{immersed_length_edge}) and (ii) the $M_k$ curve segment bases $\set{\vfedge^\ifaceapprox_{k,m}}=\set{\brackets{\vx^\ifaceapprox_{k,2m-1},\vx^\ifaceapprox_{k,2m}}}$ introduced before, whose arrangement was described in subsection~\ref{subsec:topological_connectivity}. %
\item The \textbf{non-polygonal} part can be computed efficiently resorting to the principal transformation introduced in subsection~\ref{subsec:transformation_principal_coordinates}%
; cf.~\reffig{face_decomposition} for an illustration. %
\end{enumerate}%
%
Note that, while the polygonal contribution $\immersedarea{k}^{\mathrm{poly}}$ is zero or positive, the non-polygonal contribution $\immersedarea{k}^{\mathrm{cap}}$ may become negative if the immersed face $\vfface_k^-$ is non-convex (as shown in the right panel of \reffig{face_decomposition}). %
%
% Polygonal part
%
\paragraph{Polygonal segment ($\immersedarea{k}^{\mathrm{poly}}$)}%
%
Applying the \textsc{Gaussian} divergence theorem to a polygon embedded in $\vfface_k$ yields %
\begin{align}
\immersedarea{k}^{\mathrm{poly}}=\frac{1}{2}\brackets*{%
\sum\limits_{m=1}^{N^\vfface_k}{\iprod{\vx_{k,m}^\vfface}{\cross{\brackets{\vx_{k,m+1}^\vfface-\vx_{k,m}^\vfface}}{\vn^\vfface_k}}\immersedlength{k}{m}}+%
\sum\limits_{m=1}^{M_k}{\iprod{\vx_{k,2m-1}^\ifaceapprox}{\cross{\brackets{\vx_{k,2m}^\ifaceapprox-\vx_{k,2m-1}^\ifaceapprox}}{\vn^\vfface_k}}}%
},%
\label{eqn:polygonal_area_computation}%
\end{align}
with the relative immersed lengths $\immersedlength{k}{m}$ from \reftab{immersed_length_edge}. %
However, recall that the computation of the area of a planar polygon in $\setR^3$ actually poses a two-dimensional problem. Following \citet{JCP_2021_fbip}, who for their part resort to the work of \citet{JGT_2002_fpaa}, we employ a projection onto one of the coordinate planes (with normal $\vn_p$ and $\iprod{\vn^\vfface_k}{\vn_p}\neq0$): %
\begin{align}
\abs{\vfface_k}=\frac{\abs{\vfface^{\mathrm{proj}}_{k,p}}}{\iprod{\vn^\vfface_k}{\vn_p}}%
\qquad\text{with}\qquad%
p\defeq\arg\max_p\abs{\iprod{\vn^\vfface_k}{\ve_p}},\label{eqn:face_area_projection}%
\end{align}
see~\reffig{coordinate_projection} for an illustration. %
In order for the projection to maintain the counter-clockwise order of the vertices (i.e., with respect to $\vn_p$), the projected coordinates must be arrangend as $\set{y,z}$ for $p=1$, $\set{z,x}$ for $p=2$ and $\set{x,y}$ for $p=3$. %
%
\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=1]{projected_face_polygon}%
\hfill%
\includegraphics[page=2]{projected_face_polygon}%
\hfill\null%
\caption{Coordinate plane projection $\vfface^{\mathrm{proj}}_{k,p}$ (cyan) of polygonal face $\vfface_k$ (blue). Note that the coordinate arrangement produces positive areas in \protect\refeqn{polygonal_area_computation} by accounting for $\operatorname{sign}\protect\iprod{\vn^\vfface_k}{\vn_p}$.}%
\label{fig:coordinate_projection}%
\end{figure}
%
Since the projection acts on $\darea$ as a scalar multiplication, one can simply substitute the three-dimensional points in \refeqn{polygonal_area_computation} with their projected counterparts, where the cross-product reduces to swapping two vector components. %
%
E.g., for a projection onto the $xy$-plane ($p=3$), \refeqn{polygonal_area_computation} becomes %
\begin{align}
% \vN_{k,m}^{\mathrm{proj}}\immersedlength{k}{m}^{\mathrm{proj}}=%
\immersedarea{k}^{\mathrm{poly}}=\frac{1}{2\iprod{\vn^\vfface_k}{\ve_3}}%
\brackets*{%
\sum\limits_{m=1}^{N^\vfface_k}{\brackets*{x^\vfface_{k,m}y^\vfface_{k,m+1}-y^\vfface_{k,m}x^\vfface_{k,m+1}}%
\immersedlength{k}{m}}%
+%
\sum\limits_{m=1}^{M_k}{\brackets*{x^\ifaceapprox_{k,2m-1}y^\ifaceapprox_{k,2m}-y^\ifaceapprox_{k,2m-1}x^\ifaceapprox_{k,2m}}}%
},%
\label{eqn:polygonal_area_computation_projected}%
\end{align}
and analogous expressions for the $xz$- and $yz$-plane are readily obtained. %
%
% Non-polygonal
%
\paragraph{Non-polygonal segment ($\immersedarea{k}^{\mathrm{cap}}$)}%
%
The parametrization of the curve segment in principal coordinates $\vu^\prime_k\fof{s}$ can be obtained from \refeqn{parametrization_curve_class}. %
We obtain %
\begin{align}%
\immersedarea{k}^{\mathrm{cap}}=%
\begin{cases}%
%elliptic
\frac{\sqrt{B_{k,1}B_{k,2}}}{2b_k}\sum\limits_{m=1}^{M_k}{s_{k,2m}^\ifaceapprox-s_{k,2m-1}^\ifaceapprox + \cos{s_{k,2m}^\ifaceapprox}\sin{s_{k,2m-1}^\ifaceapprox}-\cos{s_{k,2m-1}^\ifaceapprox}\sin{s_{k,2m}^\ifaceapprox}}&\text{elliptic},\\%
% hyperbolic
\sqrt{\frac{b_k}{4B_{k,1}}}\sum\limits_{m=1}^{M_k}{s_{k,2m-1}^\ifaceapprox\lambda_{2m}-s_{k,2m}^\ifaceapprox\lambda_{2m-1}+%
\sqrt{\frac{-b_k}{B_{k,2}}}\brackets{\rho_{2m}-\rho_{2m-1}}}&\text{hyperbolic ($+$)},\\%
% hyperbolic
\sqrt{\frac{b_k}{4B_{k,1}}}\sum\limits_{m=1}^{M_k}{s_{k,2m}^\ifaceapprox\lambda_{2m-1}-s_{k,2m-1}^\ifaceapprox\lambda_{2m}-%
\sqrt{\frac{-b_k}{B_{k,2}}}\brackets{\rho_{2m}-\rho_{2m-1}}}&\text{hyperbolic ($-$)},\\%
% parabola
\frac{B_{k,1}}{6\iprod{\va_k}{\vr_{2,k}}}\sum\limits_{m=1}^{M_k}{\brackets{s_{k,2m}^\ifaceapprox-s_{k,2m-1}^\ifaceapprox}^3}&\text{parabolic},\\%
% linear
0&\text{linear}%
\end{cases}%
\label{eqn:cap_area}%
\end{align}
with $\lambda_m\defeq\sqrt{1-\frac{B_{k,2}}{b_k}\brackets*{s_{k,m}^\ifaceapprox}^2}$ and %
$\rho_{m}\defeq\log\brackets*{\sqrt{-\frac{B_{k,2}}{b_k}}\lambda_m-\frac{B_{k,2}}{b_k}s_{k,m}^\ifaceapprox}$ for ease of notation; %
cf.~\refFig{face_intersection_elliptic_hyperbolic} for an illustration. %
\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=2]{curve_class_illustration_face}%
\hfill%
\includegraphics[page=1]{curve_class_illustration_face}%
\hfill%
\includegraphics[page=3]{curve_class_illustration_face}%
\hfill\null
\caption{Elliptic, hyperbolic and parabolic face intersection ($\vec{\nu}_k=\tensor[2]{R}_k\tensor[2]{\mu}_k$ denote the principal coordinates of face $\vfface_k$) with immersed area $\immersedarea{k}$ and cap area $\immersedarea{k}^{\mathrm{cap}}$ (hatched) from \protect\refeqn{cap_area}.}%
\label{fig:face_intersection_elliptic_hyperbolic}%
\end{figure}


==> 03_numerical_results.tex <==
%
% Numerical results
%
\section{Numerical results}\label{sec:numerical_results}%
In order to assess the proposed algorithm, the present section conducts a two-component series of numerical experiments. %
%
% global error
%
Firstly, we investigate various combinations of hypersurfaces and mesh types in subsection~\ref{subsec:results_global}. As a measure for accuracy, we employ the global volume error %
\begin{align}
\error_V\defeq\abs*{1-\frac{\sum_{i=1}^{\Niface}{\abs{\cell*_i\alpha_i}}}{V_\iface}},%
\label{eqn:global_volume_error}%
\end{align}
where $V_\iface=\abs{\set{\vx\in\setR^3:\lvlset_\iface\fofx\leq0}}$ and $\Niface$ denote the volume enclosed by the hypersurface $\iface$ and the number of intersected cells, respectively. %
%
The approximation error of the original volume integral in \refeqn{volume_computation_facebased_approx} comprises two distinguishable sources: (i) the approximation of the hypersurface ($\iface\to\ifaceapprox$; cf.~\refnote{approximation_quality}) and (ii) the numerical approximation (i.e., quadrature) of the resulting curve integral in \refeqn{quadrature_line_integral}. The latter can be reduced to insignifcance by choosing a sufficiently large order for the employed \textsc{Gauss-Legendre} quadrature. %
%
\begin{note}[Quadrature]%
In an extensive set of preliminary numerical experiments, we have found that the accuracy of the volume fractions does not profit from increasing $N_{\mathrm{quad}}$ beyond $5$. However, a higher number of quadrature nodes might be needed to accurately approximate general integrals of type $\int_{\iface}{\iprod{\vf}{\nS}\darea}$. %
\end{note}
%
Hence, the approximation quality of the hypersurface constitutes the limiting factor: %
from the locally quadratic approximation of the hypersurface one can expect third-order convergence with spatial resolution, corresponding to the number of intersected cells $\Niface$, which is not an input parameter. %
Recalling that $\iface$ is of codimension one with respect to the domain $\domain$ implies that $\Niface\propto N_\domain^{\frac{2}{3}}$ or, alternatively,  $\sqrt{\Niface}\propto N_\domain^{\frac{1}{3}}$. With $N_\domain^{\frac{1}{3}}$ resembling the equivalent resolution per spatial direction, we choose $\sqrt{\Niface}$ as the corresponding interface resolution. %

%
% non-convex cells
%
Secondly, note that the meshes under consideration are composed of standard convex polyhedra, which are of high relevance for productive simulations. Hence, in order to show the full capability of the proposed algorithm, subsection~\ref{subsec:results_nonconvex} exemplarily investigates a non-convex polyhedron intersected by a family of paraboloids. %

%
% Hypersurfaces
%
\subsection{Hypersurfaces}\label{subsec:experiments_hypersurfaces}%
\paragraph{Spheres and ellipsoids}%\label{subsubsec:experiments_sphere}%
In this work, we consider a sphere of radius $R_0=\frac{4}{5}$ %
as well as a prolate (semiaxes $\set{\nicefrac{3}{4},\nicefrac{1}{2},\nicefrac{1}{4}}$) and an oblate (semiaxes $\set{\nicefrac{4}{5},\nicefrac{4}{5},\nicefrac{2}{5}}$) ellipsoid, all centered at $\vx_0=\vec{0}$. %
%
% Perturbed spheres
%
\paragraph{Perturbed spheres}%
Perturbed spheres can be parametrized in spherical coordinates as %
\begin{align}
\iface=\set{\vx_0+R\fof{\varphi,\theta}\ve_r:\fof{\varphi,\theta}\in\unitsphere}%
\quad\text{with}\quad%
R\fof{\varphi,\theta;\vciface}=\brackets*{\sum\limits_{l=0}^{\Liface}{\sum\limits_{m=-l}^{l}{\ciface{lm}\sphericalharm{}}}}^{\!\frac{1}{3}},%
\end{align}
where the description of the radius $R$ employs tesseral spherical harmonics up to and including order $\Liface\in\setN$. %
The reason for expanding the third power of the radius instead of the radius itself is that the computation of the enclosed volume is considerably simplified, because $V_\iface=\ciface{00}\nicefrac{\sqrt{4\pi}}{3}$ then. %
The $(\Liface+1)^2$ coefficients $\ciface{lm}\sim\mathcal{N}(0,\sigma_0)$ are computed by the method of \citet{AMS_1958_anot}, i.e.
\begin{align}
\ciface{lm}=%
\begin{cases}
\sqrt{4\pi}R_0^3&l=0,\\%
\sqrt{\sigma_0}\sqrt{-2\log\gamma_1}\cos(2\pi\gamma_2)&l>0,%
\end{cases}\qquad\text{with}\qquad\gamma_{1,2}\sim\mathcal{U}(0,1),%
\end{align}
where the uniformly distributed numbers $\gamma_{1,2}$ are generated by the intrinsic \texttt{fortran} subroutine \texttt{random\_number()}. %
%
In this work, we consider perturbed spheres with base radius $R_0=\nicefrac{4}{5}$, modes $\Liface\in\set{3,6}$ and variance $\sigma_0=\num{5e-4}$; cf.~\reffig{hypersurface_illustration} for an illustration. %
\begin{figure}[htbp]%
\null\hfill%
\includegraphics[bb=0 0 1190 1100,height=4cm]{glsa_L3_illustration}%
\includegraphics[page=1,height=4cm]{colorcurvature}%
\hfill%
\includegraphics[bb=0 0 1190 1100,height=4cm]{glsa_L6_illustration}%
\includegraphics[page=2,height=4cm]{colorcurvature}%
\hfill%
\includegraphics[bb=0 0 1190 1100,height=4cm]{prolate_illustration}%
\includegraphics[page=3,height=4cm]{colorcurvature}%
% \hfill%
% \includegraphics[bb=0 0 1190 1100,height=3cm]{oblate_illustration}%
% \includegraphics[page=4,height=3cm]{colorcurvature}%
\hfill\null%
\caption{Illustration of perturbed spheres ($R_0=\nicefrac{4}{5}$, $\Liface=\protect\set{3,6}$ and $\sigma_0=\num{5e-4}$) and prolate ellipsoid, where the color indicates the curvature $\curv_\iface=\curv_1+\curv_2$.}%
\label{fig:hypersurface_illustration}%
\end{figure}
%
% Meshes
%
\subsection{Meshes}\label{subsec:meshes}%
In what follows, we consider the domain $\domain=[-1,1]^3$, which is decomposed into cubes of equal size and tetrahedra. The latter are generated using the library \texttt{gmsh}, introduced in the seminal paper of \citet{IJNME_2009_gmsh}. For the purpose of the present paper, however, we only resort to some of the basic features of \texttt{gmsh}; cf.~\refapp{gmsh} and \reftab{mesh_characteristics} for further details. %

\begin{table}[htbp]%
\caption{Mesh characteristics.}%
\label{tab:mesh_characteristics}%
\null\hfill%
\subtable[Tetrahedron meshes; cf.~\refapp{gmsh}.]{%
\label{tab:tetrahedron_mesh_setup}%
\begin{tabular}{c|c|c}%
\textbf{resolution}&\textbf{char. length}&\# of cells\\%&\# of faces\\%
$N$&$h=\nicefrac{1}{N}$&$N_\domain$\\%
\hline%
\num{10}&$\num{1.00e-1}$&\num{4764}\\%&\num{10261}\\%
\num{15}&$\num{6.66e-2}$&\num{15266}\\%&\num{32160}\\%
\num{20}&$\num{5.00e-2}$&\num{33744}\\%&\num{70322}\\%
\num{25}&$\num{4.00e-2}$&\num{64165}\\%&\num{132750}\\%
\num{30}&$\num{3.33e-2}$&\num{108582}\\%&\num{223550}\\%
\num{35}&$\num{2.85e-2}$&\num{171228}%&\num{351057}%
\end{tabular}%
}%
%
\hfill%
%
\subtable[Equidistant cube meshes.]{%
\label{tab:cube_mesh_setup}%
\begin{tabular}{c|c|c}%
\textbf{resolution}&\textbf{char. length}&\# of cells\\%&\# of faces\\%
$N$&$h=\frac{1}{N}$&$N_\domain=N^3$\\%&$3N^2(N+1)$\\%
\hline%
%for i in {15,20,25,70};do echo "\num{$i}&\num{"$(printf %.2e\\n "$((10000/$i))e-4")"}&\num{"$(( $i*$i*$i))"}&\num{"$(( 3*$i*($i+1)*$i ))"}\\\%";done
\num{15}&\num{6.66e-02}&\num{3375}\\%&\num{10800}\\%
\num{20}&\num{5.00e-02}&\num{8000}\\%&\num{25200}\\%
\num{25}&\num{4.00e-02}&\num{15625}\\%&\num{48750}\\%
$\vdots$&$\vdots$&$\vdots$\\%&$\vdots$\\%
\num{70}&\num{1.42e-02}&\num{343000}\\%&\num{1043700}\\%
\end{tabular}%
}%
\hfill\null%
\end{table}%
%
%
%
\subsection{Results I -- Meshes with convex cells}\label{subsec:results_global}%
\refFig{volerror_convergence} gathers the volume errors from \refeqn{global_volume_error} obtained for the hypersurfaces and meshes given in subsections~\ref{subsec:experiments_hypersurfaces} and \ref{subsec:meshes}, respectively. %
%
\begin{figure}[htbp]
\null\hfill%
\subfigure[equidistant cube]{\includegraphics[page=1]{volerror_initialization}}%
\hfill%
\subfigure[tetrahedron]{\includegraphics[page=2]{volerror_initialization}}%
\hfill\null%
\label{fig:volerror_convergence}%
\caption{Global relative volume error from \protect\refeqn{global_volume_error} as a function of intersected cells $N_\iface$ for different hypersurfaces (centered at $\vx_0=\vec{0}$ in ${\domain=[-1,1]^3}$; cf.~subsection~\ref{subsec:experiments_hypersurfaces} and \protect\reffig{hypersurface_illustration}) and meshes (cf.~\protect\reftab{mesh_characteristics}). The number of dots in the dashed lines corresponds to the order of convergence.}%
\end{figure}%

The main observations can be summarized as follows: %
\begin{enumerate}
\item As expected, the global relative volume error exhibits at least third-order convergence with spatial resolution for all combinations of hypersurfaces and meshes under consideration. %
\item For spheres, one obtains fourth-order convergence for both tetrahedral and hexahedral meshes. The rationale behind this phenomenon emerges from considering the approximation quality of the height function in \refeqn{hypersurface_approximation_quadratic}: for general hypersurfaces, the quadratic approximation in a tangential coordinate system exhibits third-order. Due to the symmetry, however, the general remainder $\hot{\norm{\vt}^3}$ effectively becomes $\hot{\norm{\vt}^4}$, which directly translates to an increased order of convergence. %
\item While the error obviously decreases with increasing spatial resolution, it is virtually independent of the underlying mesh, indicating the robustness of the proposed method. %
%
\item For comparison, \reffig{volerror_convergence} also contains the volume errors obtained from linear hypersurface approximation ($\curv_i\defeq0$). For both cube and tetrehedral meshes, the error differs between two and four orders of magnitude, which is in accordance with the findings of \citet{JCP_2019_haco}. Note that, while we only show the results for the sphere, they can be considered prototypical for the other hypersurfaces under consideration. However, owing to the approximation quality discussed above, one obtains a reduced difference (two to three) in the order of magnitude. %
%
\item For cube meshes, the results virtually coincide with those of \citet{JCP_2019_haco}. Due to the strong similarity in concept, this is to be expected. However, recall that the proposed method is applicable to unstructured meshes composed of arbitrary polyhedra, whereas the original algorithm of \citet{JCP_2019_haco} is restricted to (i) convex polyhedral cells enclosing (ii) simply connected hypersurface patches. %
\end{enumerate}%
%
%
%
\subsection{Results II -- Single non-convex polyhedron}\label{subsec:results_nonconvex}%
The previous subsection~\ref{subsec:results_global} was devoted to the investigation of general hypersurfaces intersecting hexahedral and tetrahedral (i.e., convex) meshes, highlighting the influence of hypersurface approximation; cf.~\refnote{approximation_quality}. In addition, the present section focusses on the volume computation for a given family of paraboloids intersecting a single non-convex polyhedron; cf.~\refapp{nonconvex_polyhedron} for details. %
%
%
%
\paragraph{A family of paraboloids}%
For a given base point $\xref$, base system $\set{\vn_0,\vtau}$ and curvature tensor $\curvtensor$, extending \refeqn{ifaceapprox_map} by a shift in the direction of the base normal $\vn_0$ yields a family of paraboloids, namely %
\begin{align}
\set{\ifaceapprox}_{s\in[s_{\mathrm{min}},s_{\mathrm{max}}]}=\set{\vf_\ifaceapprox\fof{\vt;s}:(\vt,s)\in\setR^2\times[s_{\mathrm{min}},s_{\mathrm{max}}]}%
\quad\text{with}\quad%
\vf_\ifaceapprox\fof{\vt;s}=\xref+\vtau\vt+\brackets{\happrox\fof{\vt}+s}\vn_0,%
\tag{\ref*{eqn:ifaceapprox_map}$^\prime$}%
\label{eqn:shifted_paraboloid}%
\end{align}
where the associated level-set analogously extends \refeqn{ifaceapprox_lvlset}. %
As for the parameters of the paraboloid, we choose %
\begin{align}%
\xref=\frac{\brackets*[s]{1,1,1}\transpose}{2},\quad%
\vn_0=\frac{\brackets*[s]{4,-7,2}\transpose}{\sqrt{69}},\quad%
\vtau_1=\frac{\brackets*[s]{-8,14,65}\transpose}{\sqrt{4485}},\quad
\vtau_2=\frac{\brackets*[s]{-7,-4,0}\transpose}{\sqrt{65}},\quad%
\curv_1=-\frac{19}{4}\quad\text{and}\quad%
\curv_2=0.%
\label{eqn:paraboiloid_parameters}%
\end{align}
The left panel in \reffig{illustration_graphbase} illustrates the intersection with a unit cube for $s=0$. %
%
\begin{remark}[Choice of parameters]%
Recall from \reftab{possible_curve_class} that there are four classes of boundary curves: hyperbolic, elliptic, parabolic and linear. %
The first two require (i) non-zero \textsc{Gaussian} curvature as well as (ii) non-orthogonality of the containing face $\vfface_k$ and the base plane of the paraboloid, i.e.~$\iprod{\vn^\vfface_k}{\vn_0}\neq0$. Complementary, parabolic curve segments may emerge if either (i) one of the principal curvatures $\curv_i$ is zero for $\iprod{\vn^\vfface_k}{\vn_0}\neq0$ or (ii) $\iprod{\vn^\vfface_k}{\vn_0}=0$ for arbitrary values of $\curv_i$.
Hence, due to the choice of the hypersurfaces in subsection~\ref{subsec:experiments_hypersurfaces}, in statistical terms, one cannot expect to encounter parabolic or linear boundary curve segments. %
Therefore, the present subsection aims at examining parabolic and linear curve segments by purposely setting one of the principal curvatures, say $\curv_2$, to zero. %
\end{remark}%
%
The boundaries of the shift interval are chosen to ensure that $\polyvof\fof{s_{\mathrm{min}}}=0$ and $\polyvof\fof{s_{\mathrm{max}}}=1$, i.e.~such that the volume fraction
\begin{align}
\polyvof\fof{s}=\abs{\cell*}^{-1}\abs{\set{\vx\in\cell*:\lvlset_\ifaceapprox\fof{\vx;s}\leq0}}%
\label{eqn:nonconvex_volume_fraction}%
\end{align}
traverses all possible values. Here, let $s_{\mathrm{min}}\defeq-1$ and $s_{\mathrm{max}}\defeq\nicefrac{3}{2}$. %
It is worth noting that, for non-degenerate\footnote{\citet[Section~2]{JCP_2021_fbip} consider the regularity of planar $\ifaceapprox$ for intersection with convex and non-convex polyhedra.} paraboloids ($\curv_i\neq0$), the function $\polyvof:\setR\mapsto[0,1]$ is strictly monotonous and continuously differentiable. The regularity in the degenerate case (at least one trivial principal curvature) depends on the topological properties of the polyhedron as well as the paraboloid parameters. %
%
\begin{remark}[Partial derivative]%
After replacing $\iface$ with $\ifaceapprox$ in \refeqn{volume_computation} and applying the \textsc{Reynolds} transport theorem, it is easy to show that %
$\abs{\cell*}\partial_s\polyvof\fof{s}=\int_{\ifaceapprox}{\iprod{\partial_s\vf_\ifaceapprox}{\vn_\ifaceapprox}\darea}=\abs{\support_\ifaceapprox}\geq0$, %
i.e.~the derivative of the volume fraction with respect to the base normal shift parameter corresponds to the area of the graph base $\support_\ifaceapprox$. For planar paraboloids, one trivially obtains $\abs{\support_\ifaceapprox}=\abs{\ifaceapprox\cap\cell*}$, which can be exploited, e.g., for efficient PLIC interface positioning schemes \cite{XXX_2020_ivof,JCP_2021_fbip,JCP_2021_etmp}. % or \citet[eq.~(30)]{JCP_2019_apnm}. %
\end{remark}
%
\refFig{nonconvex_volume_fraction} depicts the volume fraction $\polyvof$ and its derivative with respect to the shift parameter $s$ as a function of the latter, where \reffig{nonconvex_volume_fraction_illustration} illustrates some of the intersections. %
%
\begin{figure}[htbp]%
\null\hfill%
\includegraphics{nonconvex_volume_fraction}%
\hfill\null%
\caption{Volume fractions $\polyvof$ from \protect\refeqn{nonconvex_volume_fraction} induced by the family of paraboloids given in \protect\refeqn{shifted_paraboloid} as a function of the normalized shift $s$ with ${[s_{\mathrm{min}},s_{\mathrm{max}}]=[-1,\nicefrac{3}{2}]}$.}%
\label{fig:nonconvex_volume_fraction}%
\end{figure}%

\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=1]{nonconvex_example}%
\hfill%
\includegraphics[page=1]{nonconvex_boundarycurve_paradom}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=2]{nonconvex_example}%
\hfill%
\includegraphics[page=2]{nonconvex_boundarycurve_paradom}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=3]{nonconvex_example}%
\hfill%
\includegraphics[page=3]{nonconvex_boundarycurve_paradom}%
\hfill\null%
\caption{Polyhedron "table" intersected by shifted paraboloid (blue shade: $\ifaceapprox\cap\protect\cell*$) given in \protect\refeqn{shifted_paraboloid} with associated graph base $\support_\ifaceapprox$ at normalized positions $\nicefrac{1}{4}$, $\nicefrac{2}{5}$ and $\nicefrac{39}{50}$ (corresponding to the vertical dashed lines in \protect\reffig{nonconvex_volume_fraction}) in interval ${[s_{\mathrm{min}},s_{\mathrm{max}}]=[-1,\nicefrac{3}{2}]}$.}%
\label{fig:nonconvex_volume_fraction_illustration}%
\end{figure}


==> 04_conclusion.tex <==
\section{Conclusion \& Outlook}\label{sec:conclusion}%
We have introduced an algorithm for the computation of volumes induced by a intersection of a paraboloid with an arbitrary polyhedron, where the paraboloid parameters are obtained from a locally quadratic approximation of a given hypersurface. %
The recursive application of the \textsc{Gaussian} divergence theorem in its respectively appropriate form allows for a highly efficient face-based computation of the volume of the truncated polyhedron, implying that no connectivity information has to be established at runtime. Furthermore, the face-based character renders the presented approach most suitable for parallel computations on unstructured meshes. %
%
A classification of the boundary curve segments $\partial\ifaceapprox_k$ associated to the polyhedron faces $\vfface_k$ allows for their explicit parametrization, which has been shown to be favourable for the computation of quadrature nodes and weights. This in turn greatly facilitates the approximation of the associated curve integrals. %
We have conducted a twofold assessment of our algorithm: %
firstly, by examining convex meshes with different hypersurfaces, resemebling a commonly encountered task for obtaining the initial configuration of two-phase flow simulations. For each cell, the paraboloid parameters are obtained from a locally quadratic approximation based on the level-set of the original hypersurface. %
The global volume errors show the expected third- to fourth-order convergence with spatial resolution, along with a reduction of about 2 orders of magnitude in comparison to linear approximation. %
%
Secondly, by intersecting a paramterized family of paraboloids with an exemplary non-convex polyhedron, which serves to illustrate the capability of the proposed algorithm. %
%

Altogether, we draw the following conclusions: %
\begin{enumerate}%
\item The recursive application of the \textsc{Gaussian} divergence theorem in appropriate form allows for an efficient computation of the volume of a truncated \textbf{arbitrary polyhedron}. This face-based problem decomposition allows to \textbf{avoid extracting topological connectivity}, which is advantageous in terms of implementation complexity, computational effort and parallelization. %
\item The quadrature nodes and weights can easily be employed to evaluate general integrals of type $\int_{\ifaceapprox}{\iprod{\vf}{\vn_\ifaceapprox}\darea}$ for integrands $\vf$ which are polynomial in the spatial coordinate $\vx$. Note that, e.g., the partial derivatives of the volume with respect to the paraboloid parameters can be written in this form. In fact, the present algorithm constitutes an important building block for a generalization of the parabolic reconstruction of interfaces from volume fractions, originally proposed for structured hexahedral grids by \citet{JCP_2002_prost}. %
\end{enumerate}%

